Bi-Fact: A Bidirectional Factorization-based Evaluation of Intent Extraction from UI Trajectories

Evaluating intent extraction from GUIs demands accurate, fine-grained metrics. This paper introduces Bi-Fact, a novel method that decomposes intents into atomic facts and performs bidirectional comparisons to assess precision and recall. Experiments demonstrate Bi-Fact's superior correlation with human judgments compared to existing metrics, establishing a more robust evaluation framework for UI-driven intent understanding.

==> sections/dataset.tex <==

\subsection{Dataset and Annotation}

We annotated a dataset of intent pairs (gold and predicted) labeling whether they are likely to produce similar UI trajectories and achieve the same goal.  Examples include "Play the top rated movie" vs. "Play The Shawshank Redemption" (different trajectories) and "Show top rated hotels" vs. "Show 5 star rated hotels" (similar trajectories).  A smaller dataset was also labeled for fact correctness. The full dataset has 2000 examples, annotated by 6 raters with a consolidated optimal label. 1000 examples have a consolidated label based on 7 labels (6 raters + scratch), and another 1000 examples have a consolidated label based on 6 raters. Out of these, 138 examples have expert annotation (Tal).

\section{Data Contribution}

We contribute a higher-quality subset of SCRATCH, based on manual annotation, and an improved, automatically cleaned version.  We provide detailed annotation guidelines and methodology, especially for cases where gold intents are not available upfront.  We also explore synthetic gold generation via automatic consolidation.


\subsection{Evaluation Methodology}

We evaluate AutoFact in two main experiments:

\subsubsection{Experiment 1: Evaluation Methodology}

We compare AutoFact to other metrics using a full-match labeled dataset. We compare AutoEval Full Match prompt, double-sided NLI, and AutoFact using F1-score and AUC-ROC.

\subsubsection{Experiment 2: Optimal Annotation Strategy}

We evaluate AutoFact's performance on datasets with different annotation strategies: cleaned Scratch, annotations from individual raters, single prompt optimal annotation, pyramid method, Socratic method, self-critique, 3 random raters, and the best 3 raters.


==> sections/prior_work.tex <==

\section{Prior Work}

Intent understanding and comparison have been widely studied in natural language processing (NLP) and human-computer interaction (HCI). Traditional approaches rely on text similarity metrics such as BLEU \cite{papineni2002bleu} and ROUGE \cite{lin2004rouge}, which measure lexical overlap but struggle to capture semantic equivalence. More advanced embedding-based methods, such as BERTScore \cite{zhang2019bertscore}, improve upon this by leveraging contextualized representations, though they may still fail to distinguish functional differences in intent.

Beyond text-based methods, Natural Language Inference (NLI) models \cite{bowman2015large} have been employed to determine logical relationships between intents, but their effectiveness in UI-based intent comparison remains limited. Recent work has also introduced \textit{automated evaluation frameworks} \cite{berkovitch2024identifying} that leverage heuristic and learned scoring methods to assess intent similarity, though challenges remain in aligning automated metrics with human judgments.

In UI-based tasks, datasets like Mind2Web \cite{mind2web2024} and AitW \cite{aitw2024} provide benchmarks for evaluating agent performance in structured web and mobile environments. However, comparing intents within these datasets remains an open challenge, as standard NLP metrics fail to capture the nuances of user trajectories and execution paths. Our work builds upon these efforts by introducing a more structured, fact-based comparison metric designed specifically for downstream UI automation and memory-based retrieval tasks.

